Near-circular orbits for planets around M/K-type stars with Earth-like sizes and instellations

Recent advances have enabled the discovery of a population of potentially Earth-like planets, yet their orbital eccentricity, which governs their climate and provides clues about their origin and dynamical history, is still largely unconstrained. We identify a sample of 17 transiting exoplanets around late-type stars with similar radii and irradiation to that of Earth and use the "photoeccentric effect" - which exploits transit durations - to infer their eccentricity distribution via hierarchical Bayesian modelling. Our analysis establishes that these worlds further resemble Earth in that their eccentricities are nearly circular (mean eccentricity $=0.060_{-0.028}^{+0.040}$ and $\leq0.15$), with the exception of one outlier of moderate eccentricity. The results hint at a subset population of dynamically warmer Earths, but this requires a larger sample to statistically confirm. The planets in our sample are thus largely subject to minimal eccentricity-induced seasonal variability and are consistent with emerging via smooth disk migration rather than violent planet-planet scattering.

==> tables/toi1266_02.tex <==
\begin{table*}
\caption{Transit times for TOI-1266.02. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
-49 & $1689.967\pm0.017$ & $11.\pm11.$ \\
-47 & $1727.564\pm0.0078$ & $1.\pm1.$ \\
-39 & $1877.9772\pm0.0082$ & $1.\pm1.$ \\
-38 & $1896.7758\pm0.0078$ & $-4.\pm-4.$ \\
-10 & $2423.2337\pm0.0065$ & $11.5\pm11.5$ \\
-9 & $2442.0216\pm0.0042$ & $-8.3\pm-8.3$ \\
0 & $2611.2479\pm0.0056$ & $7.5\pm7.5$ \\
1 & $2630.0432\pm0.0051$ & $-1.7\pm-1.7$ \\
\hline\hline
\end{tabular}
\label{tab:1266_02} % is used to refer this table in the text
\end{table*}

==> tables/toi1452_01.tex <==
\begin{table*}
\caption{Transit times for TOI-1452.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1691.533\pm0.016$ & $-3.\pm-3.$ \\
1 & $1702.6\pm0.012$ & $4.\pm4.$ \\
2 & $1713.649\pm0.023$ & $-14.\pm-14.$ \\
4 & $1735.82\pm0.048$ & $54.\pm54.$ \\
5 & $1746.8439\pm0.0085$ & $-1.\pm-1.$ \\
6 & $1757.9107\pm0.0097$ & $6.\pm6.$ \\
7 & $1768.9649\pm0.0079$ & $-5.\pm-5.$ \\
8 & $1780.0326\pm0.0071$ & $3.\pm3.$ \\
12 & $1824.283\pm0.01$ & $7.\pm7.$ \\
13 & $1835.341\pm0.041$ & $2.\pm2.$ \\
14 & $1846.396\pm0.037$ & $-9.\pm-9.$ \\
15 & $1857.465\pm0.016$ & $1.\pm1.$ \\
16 & $1868.528\pm0.019$ & $3.\pm3.$ \\
17 & $1879.586\pm0.01$ & $-2.\pm-2.$ \\
18 & $1890.645\pm0.015$ & $-8.\pm-8.$ \\
19 & $1901.707\pm0.012$ & $-7.\pm-7.$ \\
21 & $1923.841\pm0.011$ & $8.\pm8.$ \\
22 & $1934.883\pm0.029$ & $-21.\pm-21.$ \\
24 & $1957.023\pm0.011$ & $2.\pm2.$ \\
25 & $1968.095\pm0.015$ & $16.\pm16.$ \\
26 & $1979.146\pm0.011$ & $1.\pm1.$ \\
27 & $1990.211\pm0.012$ & $6.\pm6.$ \\
28 & $2001.262\pm0.014$ & $-10.\pm-10.$ \\
29 & $2012.3342\pm0.0085$ & $4.\pm4.$ \\
30 & $2023.3892\pm0.0078$ & $-6.\pm-6.$ \\
31 & $2034.455\pm0.011$ & $0.\pm0.$ \\
64 & $2399.493\pm0.0085$ & $-9.\pm-9.$ \\
65 & $2410.5523\pm0.0096$ & $-12.\pm-12.$ \\
66 & $2421.616\pm0.02$ & $-10.\pm-10.$ \\
67 & $2432.711\pm0.052$ & $38.\pm38.$ \\
68 & $2443.729\pm0.011$ & $-26.\pm-26.$ \\
81 & $2587.5593\pm0.0052$ & $10.8\pm10.8$ \\
82 & $2598.6134\pm0.006$ & $-0.6\pm-0.6$ \\
\hline\hline
\end{tabular}
\label{tab:1452_01} % is used to refer this table in the text
\end{table*}

==> tables/toi2079_02.tex <==
\begin{table*}
\caption{Transit times for TOI-2079.02. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
-97 & $1729.8745\pm0.0092$ & $8.\pm8.$ \\
-78 & $1906.8913\pm0.0044$ & $-13.\pm-13.$ \\
-76 & $1925.544\pm0.0047$ & $12.7\pm12.7$ \\
-22 & $2428.6989\pm0.0069$ & $31.3\pm31.3$ \\
-21 & $2437.9861\pm0.0042$ & $-12.3\pm-12.3$ \\
-2 & $2615.049\pm0.043$ & $33.\pm33.$ \\
0 & $2633.6611\pm0.0041$ & $0.2\pm0.2$ \\
\hline\hline
\end{tabular}
\label{tab:2079_02} % is used to refer this table in the text
\end{table*}

==> tables/toi2093_01.tex <==
\begin{table*}
\caption{Transit times for TOI-2093.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1751.629\pm0.016$ & $18.\pm18.$ \\
1 & $1805.419\pm0.012$ & $-11.\pm-11.$ \\
2 & $1859.241\pm0.014$ & $4.\pm4.$ \\
4 & $1966.864\pm0.019$ & $6.\pm6.$ \\
12 & $2397.334\pm0.012$ & $-19.\pm-19.$ \\
16 & $2612.5934\pm0.0059$ & $3.6\pm3.6$ \\
\hline\hline
\end{tabular}
\label{tab:2093_01} % is used to refer this table in the text
\end{table*}

==> tables/toi2094_01.tex <==
\begin{table*}
\caption{Transit times for TOI-2094.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1691.309\pm0.052$ & $-33.\pm-33.$ \\
1 & $1710.134\pm0.017$ & $16.\pm16.$ \\
2 & $1728.917\pm0.013$ & $3.\pm3.$ \\
3 & $1747.697\pm0.02$ & $-13.\pm-13.$ \\
4 & $1766.492\pm0.016$ & $-8.\pm-8.$ \\
7 & $1822.867\pm0.018$ & $-9.\pm-9.$ \\
9 & $1860.456\pm0.012$ & $0.\pm0.$ \\
10 & $1879.2481\pm0.0098$ & $0.\pm0.$ \\
12 & $1916.824\pm0.02$ & $-10.\pm-10.$ \\
13 & $1935.623\pm0.064$ & $1.\pm1.$ \\
14 & $1954.419\pm0.016$ & $7.\pm7.$ \\
15 & $1973.24\pm0.024$ & $50.\pm50.$ \\
16 & $1992.001\pm0.023$ & $5.\pm5.$ \\
17 & $2010.785\pm0.015$ & $-6.\pm-6.$ \\
18 & $2029.551\pm0.031$ & $-42.\pm-42.$ \\
\hline\hline
\end{tabular}
\label{tab:2094_01} % is used to refer this table in the text
\end{table*}

==> tables/toi2095_01.tex <==
\begin{table*}
\caption{Transit times for TOI-2095.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1692.833\pm0.043$ & $44.\pm44.$ \\
2 & $1728.138\pm0.036$ & $10.\pm10.$ \\
3 & $1745.789\pm0.028$ & $-10.\pm-10.$ \\
5 & $1781.134\pm0.018$ & $13.\pm13.$ \\
6 & $1798.798\pm0.016$ & $13.\pm13.$ \\
7 & $1816.449\pm0.021$ & $-8.\pm-8.$ \\
8 & $1834.12\pm0.016$ & $1.\pm1.$ \\
9 & $1851.759\pm0.035$ & $-35.\pm-35.$ \\
11 & $1887.121\pm0.067$ & $12.\pm12.$ \\
12 & $1904.765\pm0.013$ & $-18.\pm-18.$ \\
13 & $1922.471\pm0.021$ & $42.\pm42.$ \\
14 & $1940.098\pm0.019$ & $-13.\pm-13.$ \\
15 & $1957.796\pm0.035$ & $36.\pm36.$ \\
16 & $1975.415\pm0.015$ & $-31.\pm-31.$ \\
18 & $2010.778\pm0.014$ & $18.\pm18.$ \\
19 & $2028.425\pm0.019$ & $-7.\pm-7.$ \\
53 & $2629.03\pm0.016$ & $5.\pm5.$ \\
\hline\hline
\end{tabular}
\label{tab:2095_01} % is used to refer this table in the text
\end{table*}

==> tables/toi2095_02.tex <==
\begin{table*}
\caption{Transit times for TOI-2095.02. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1704.248\pm0.033$ & $-50.\pm-50.$ \\
1 & $1732.458\pm0.038$ & $4.\pm4.$ \\
2 & $1760.653\pm0.028$ & $35.\pm35.$ \\
4 & $1816.986\pm0.019$ & $15.\pm15.$ \\
5 & $1845.136\pm0.031$ & $-19.\pm-19.$ \\
6 & $1873.342\pm0.021$ & $29.\pm29.$ \\
7 & $1901.472\pm0.04$ & $-33.\pm-33.$ \\
9 & $1957.813\pm0.03$ & $-41.\pm-41.$ \\
11 & $2014.175\pm0.025$ & $-19.\pm-19.$ \\
25 & $2408.622\pm0.016$ & $11.\pm11.$ \\
26 & $2436.776\pm0.019$ & $-17.\pm-17.$ \\
32 & $2605.832\pm0.017$ & $6.\pm6.$ \\
\hline\hline
\end{tabular}
\label{tab:2095_02} % is used to refer this table in the text
\end{table*}

==> tables/toi2285_01.tex <==
\begin{table*}
\caption{Transit times for TOI-2285.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1747.18\pm0.013$ & $1.\pm1.$ \\
1 & $1774.449\pm0.012$ & $-1.\pm-1.$ \\
8 & $1965.3398\pm0.0077$ & $0.\pm0.$ \\
\hline\hline
\end{tabular}
\label{tab:2285_01} % is used to refer this table in the text
\end{table*}

==> tables/toi2322_01.tex <==
\begin{table*}
\caption{Transit times for TOI-2322.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
-17 & $2037.428\pm0.01$ & $12.\pm12.$ \\
-16 & $2057.6428\pm0.0083$ & $-3.\pm-3.$ \\
-15 & $2077.8738\pm0.0094$ & $6.\pm6.$ \\
-14 & $2098.083\pm0.01$ & $-18.\pm-18.$ \\
-13 & $2118.295\pm0.012$ & $-37.\pm-37.$ \\
-12 & $2138.5635\pm0.01$ & $26.\pm26.$ \\
-10 & $2178.997\pm0.0088$ & $2.\pm2.$ \\
-9 & $2199.2201\pm0.0085$ & $-1.\pm-1.$ \\
-8 & $2219.44\pm0.01$ & $-8.\pm-8.$ \\
-6 & $2259.9027\pm0.0087$ & $10.\pm10.$ \\
-4 & $2300.3403\pm0.0083$ & $-9.\pm-9.$ \\
-2 & $2340.803\pm0.01$ & $9.\pm9.$ \\
0 & $2381.245\pm0.011$ & $-3.\pm-3.$ \\
\hline\hline
\end{tabular}
\label{tab:2322_01} % is used to refer this table in the text
\end{table*}

==> tables/toi237_01.tex <==
\begin{table*}
\caption{Transit times for TOI-237.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1355.2502\pm0.0051$ & $5.4\pm5.4$ \\
1 & $1360.671\pm0.0063$ & $-13.7\pm-13.7$ \\
2 & $1366.1229\pm0.0087$ & $12.\pm12.$ \\
3 & $1371.5507\pm0.0081$ & $3.\pm3.$ \\
4 & $1376.9797\pm0.0074$ & $-4.\pm-4.$ \\
135 & $2088.8346\pm0.008$ & $0.\pm0.$ \\
\hline\hline
\end{tabular}
\label{tab:237_01} % is used to refer this table in the text
\end{table*}

==> tables/toi406_01.tex <==
\begin{table*}
\caption{Transit times for TOI-406.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1388.5708\pm0.003$ & $5.4\pm5.4$ \\
1 & $1401.7418\pm0.0031$ & $-1.4\pm-1.4$ \\
2 & $1414.9131\pm0.0052$ & $-7.9\pm-7.9$ \\
3 & $1428.0924\pm0.004$ & $-2.7\pm-2.7$ \\
56 & $2126.4048\pm0.0059$ & $-5.5\pm-5.5$ \\
57 & $2139.5865\pm0.0029$ & $3.1\pm3.1$ \\
58 & $2152.7492\pm0.0074$ & $-16.\pm-16.$ \\
59 & $2165.9371\pm0.0042$ & $1.7\pm1.7$ \\
\hline\hline
\end{tabular}
\label{tab:406_01} % is used to refer this table in the text
\end{table*}

==> tables/toi5388_01.tex <==
\begin{table*}
\caption{Transit times for TOI-5388.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
\hline\hline
\end{tabular}
\label{tab:5388_01} % is used to refer this table in the text
\end{table*}

==> tables/toi5713_01.tex <==
\begin{table*}
\caption{Transit times for TOI-5713.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1745.6754\pm0.0093$ & $-5.\pm-5.$ \\
1 & $1756.1222\pm0.0083$ & $2.\pm2.$ \\
15 & $1902.3128\pm0.0098$ & $1.\pm1.$ \\
17 & $1923.2126\pm0.0092$ & $23.\pm23.$ \\
18 & $1933.629\pm0.01$ & $-14.\pm-14.$ \\
20 & $1954.509\pm0.014$ & $-22.\pm-22.$ \\
\hline\hline
\end{tabular}
\label{tab:5713_01} % is used to refer this table in the text
\end{table*}

==> tables/toi5716_01.tex <==
\begin{table*}
\caption{Transit times for TOI-5716.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
105 & $2394.078\pm0.011$ & $29.\pm29.$ \\
107 & $2407.6037\pm0.0076$ & $18.\pm18.$ \\
108 & $2414.3304\pm0.0082$ & $-40.\pm-40.$ \\
133 & $2583.5174\pm0.0079$ & $-11.\pm-11.$ \\
134 & $2590.2951\pm0.0066$ & $4.8\pm4.8$ \\
135 & $2597.051\pm0.023$ & $-11.\pm-11.$ \\
136 & $2603.789\pm0.046$ & $-52.\pm-52.$ \\
137 & $2610.523\pm0.032$ & $-99.\pm-99.$ \\
138 & $2617.3618\pm0.0095$ & $5.\pm5.$ \\
140 & $2630.908\pm0.012$ & $23.\pm23.$ \\
\hline\hline
\end{tabular}
\label{tab:5716_01} % is used to refer this table in the text
\end{table*}

==> tables/toi5728_01.tex <==
\begin{table*}
\caption{Transit times for TOI-5728.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
29 & $2018.533\pm0.023$ & $-10.\pm-10.$ \\
30 & $2030.038\pm0.04$ & $1.\pm1.$ \\
62 & $2397.982\pm0.022$ & $52.\pm52.$ \\
63 & $2409.421\pm0.017$ & $-31.\pm-31.$ \\
64 & $2420.945\pm0.02$ & $7.\pm7.$ \\
65 & $2432.446\pm0.026$ & $12.\pm12.$ \\
66 & $2443.906\pm0.046$ & $-40.\pm-40.$ \\
78 & $2581.931\pm0.016$ & $44.\pm44.$ \\
80 & $2604.899\pm0.048$ & $7.\pm7.$ \\
81 & $2616.378\pm0.01$ & $-20.\pm-20.$ \\
82 & $2627.888\pm0.015$ & $-1.\pm-1.$ \\
\hline\hline
\end{tabular}
\label{tab:5728_01} % is used to refer this table in the text
\end{table*}

==> tables/toi700_02.tex <==
\begin{table*}
\caption{Transit times for TOI-700.02. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1330.476\pm0.021$ & $-2.\pm-2.$ \\
2 & $1405.3205\pm0.0074$ & $-9.\pm-9.$ \\
3 & $1442.761\pm0.014$ & $15.\pm15.$ \\
4 & $1480.184\pm0.023$ & $13.\pm13.$ \\
6 & $1555.0242\pm0.0075$ & $0.\pm0.$ \\
7 & $1592.443\pm0.015$ & $-7.\pm-7.$ \\
9 & $1667.303\pm0.0073$ & $8.\pm8.$ \\
19 & $2041.524\pm0.015$ & $-25.\pm-25.$ \\
20 & $2078.978\pm0.025$ & $18.\pm18.$ \\
21 & $2116.3861\pm0.0044$ & $-5.5\pm-5.5$ \\
22 & $2153.851\pm0.016$ & $52.\pm52.$ \\
25 & $2266.1238\pm0.0096$ & $52.\pm52.$ \\
26 & $2303.4994\pm0.0075$ & $-18.\pm-18.$ \\
27 & $2340.9272\pm0.0096$ & $-13.\pm-13.$ \\
\hline\hline
\end{tabular}
\label{tab:700_02} % is used to refer this table in the text
\end{table*}

==> tables/toi700_04.tex <==
\begin{table*}
\caption{Transit times for TOI-700.04. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1352.1\pm0.022$ & $-8.\pm-8.$ \\
5 & $1492.057\pm0.021$ & $7.\pm7.$ \\
6 & $1519.807\pm0.026$ & $-79.\pm-79.$ \\
7 & $1547.685\pm0.024$ & $19.\pm19.$ \\
8 & $1575.522\pm0.023$ & $60.\pm60.$ \\
9 & $1603.315\pm0.023$ & $35.\pm35.$ \\
11 & $1658.891\pm0.02$ & $-26.\pm-26.$ \\
26 & $2076.006\pm0.029$ & $-64.\pm-64.$ \\
28 & $2131.686\pm0.039$ & $25.\pm25.$ \\
29 & $2159.489\pm0.031$ & $14.\pm14.$ \\
31 & $2215.082\pm0.066$ & $-22.\pm-22.$ \\
32 & $2242.907\pm0.02$ & $1.\pm1.$ \\
34 & $2298.547\pm0.035$ & $30.\pm30.$ \\
35 & $2326.344\pm0.02$ & $12.\pm12.$ \\
36 & $2354.134\pm0.021$ & $-15.\pm-15.$ \\
\hline\hline
\end{tabular}
\label{tab:700_04} % is used to refer this table in the text
\end{table*}

==> tables/toi712_04.tex <==
\begin{table*}
\caption{Transit times for TOI-712.04. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
-10 & $1385.984\pm0.03$ & $-54.\pm-54.$ \\
-9 & $1470.8594\pm0.006$ & $-3.5\pm-3.5$ \\
-8 & $1555.741\pm0.041$ & $56.\pm56.$ \\
-1 & $2149.6078\pm0.0054$ & $34.\pm34.$ \\
0 & $2234.405\pm0.0052$ & $-28.\pm-28.$ \\
1 & $2319.267\pm0.065$ & $4.\pm4.$ \\
\hline\hline
\end{tabular}
\label{tab:712_04} % is used to refer this table in the text
\end{table*}

==> tables/toi715_01.tex <==
\begin{table*}
\caption{Transit times for TOI-715.01. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1327.547\pm0.012$ & $1.\pm1.$ \\
1 & $1346.834\pm0.01$ & $0.\pm0.$ \\
2 & $1366.109\pm0.016$ & $-20.\pm-20.$ \\
4 & $1404.695\pm0.016$ & $-5.\pm-5.$ \\
6 & $1443.288\pm0.017$ & $18.\pm18.$ \\
7 & $1462.55\pm0.017$ & $-19.\pm-19.$ \\
8 & $1481.833\pm0.021$ & $-26.\pm-26.$ \\
9 & $1501.137\pm0.027$ & $-4.\pm-4.$ \\
10 & $1520.432\pm0.022$ & $6.\pm6.$ \\
11 & $1539.693\pm0.036$ & $-33.\pm-33.$ \\
13 & $1578.309\pm0.015$ & $23.\pm23.$ \\
15 & $1616.875\pm0.014$ & $10.\pm10.$ \\
16 & $1636.147\pm0.015$ & $-14.\pm-14.$ \\
17 & $1655.452\pm0.017$ & $11.\pm11.$ \\
18 & $1674.735\pm0.021$ & $2.\pm2.$ \\
37 & $2041.2092\pm0.0086$ & $2.\pm2.$ \\
41 & $2118.383\pm0.012$ & $32.\pm32.$ \\
42 & $2137.642\pm0.012$ & $-9.\pm-9.$ \\
44 & $2176.231\pm0.012$ & $9.\pm9.$ \\
45 & $2195.521\pm0.012$ & $12.\pm12.$ \\
47 & $2234.0896\pm0.008$ & $1.\pm1.$ \\
48 & $2253.374\pm0.01$ & $-5.\pm-5.$ \\
49 & $2272.659\pm0.012$ & $-9.\pm-9.$ \\
50 & $2291.9492\pm0.0096$ & $-6.\pm-6.$ \\
51 & $2311.234\pm0.012$ & $-11.\pm-11.$ \\
52 & $2330.5279\pm0.0093$ & $-3.\pm-3.$ \\
54 & $2369.091\pm0.013$ & $-22.\pm-22.$ \\
55 & $2388.402\pm0.011$ & $11.\pm11.$ \\
\hline\hline
\end{tabular}
\label{tab:715_01} % is used to refer this table in the text
\end{table*}

==> tables/toi789_02.tex <==
\begin{table*}
\caption{Transit times for TOI-789.02. Transit times are quoted as the median of the posterior and the surrounding 1-sigma interval.} % title of Table
\centering % used for centering table
\begin{tabular}{l l l}
\hline\hline %inserts double horizontal lines
Epoch & $\tau_i$ [BJD$_{\mathrm{UTC}}-2457000$] & TTV [mins] \\
%heading
\hline % inserts single horizontal line
0 & $1334.759\pm0.014$ & $-10.\pm-10.$ \\
1 & $1347.776\pm0.036$ & $56.\pm56.$ \\
2 & $1360.697\pm0.035$ & $-15.\pm-15.$ \\
3 & $1373.642\pm0.03$ & $-52.\pm-52.$ \\
4 & $1386.692\pm0.039$ & $62.\pm62.$ \\
5 & $1399.663\pm0.037$ & $62.\pm62.$ \\
8 & $1438.553\pm0.049$ & $31.\pm31.$ \\
9 & $1451.452\pm0.044$ & $-73.\pm-73.$ \\
17 & $1555.249\pm0.055$ & $-28.\pm-28.$ \\
18 & $1568.253\pm0.056$ & $20.\pm20.$ \\
19 & $1581.212\pm0.036$ & $4.\pm4.$ \\
20 & $1594.211\pm0.032$ & $44.\pm44.$ \\
21 & $1607.15\pm0.012$ & $-2.\pm-2.$ \\
22 & $1620.124\pm0.016$ & $3.\pm3.$ \\
23 & $1633.094\pm0.024$ & $2.\pm2.$ \\
24 & $1646.057\pm0.018$ & $-9.\pm-9.$ \\
25 & $1659.016\pm0.047$ & $-26.\pm-26.$ \\
26 & $1672.018\pm0.021$ & $20.\pm20.$ \\
61 & $2125.98\pm0.02$ & $2.\pm2.$ \\
62 & $2138.95\pm0.015$ & $0.\pm0.$ \\
63 & $2151.937\pm0.044$ & $24.\pm24.$ \\
64 & $2164.908\pm0.02$ & $24.\pm24.$ \\
65 & $2177.884\pm0.03$ & $32.\pm32.$ \\
66 & $2190.816\pm0.016$ & $-24.\pm-24.$ \\
67 & $2203.79\pm0.015$ & $-20.\pm-20.$ \\
68 & $2216.769\pm0.014$ & $-8.\pm-8.$ \\
78 & $2346.486\pm0.061$ & $7.\pm7.$ \\
79 & $2359.486\pm0.026$ & $49.\pm49.$ \\
80 & $2372.412\pm0.03$ & $-15.\pm-15.$ \\
81 & $2385.404\pm0.026$ & $16.\pm16.$ \\
\hline\hline
\end{tabular}
\label{tab:789_02} % is used to refer this table in the text
\end{table*}
